Physically-Feasible Reactive Synthesis for Terrain-Adaptive Locomotion via Trajectory Optimization and Symbolic Repair

We propose an integrated planning framework for quadrupedal locomotion over dynamically changing, unforeseen terrains. Existing approaches either rely on heuristics for instantaneous foothold selection--compromising safety and versatility--or solve expensive trajectory optimization problems with complex terrain features and long time horizons. In contrast, our framework leverages reactive synthesis to generate correct-by-construction controllers at the symbolic level, and mixed-integer convex programming (MICP) for dynamic and physically feasible footstep planning for each symbolic transition. We use a high-level manager to reduce the large state space in synthesis by incorporating local environment information, improving synthesis scalability. To handle specifications that cannot be met due to dynamic infeasibility, and to minimize costly MICP solves, we leverage a symbolic repair process to generate only necessary symbolic transitions. During online execution, re-running the MICP with real-world terrain data, along with runtime symbolic repair, bridges the gap between offline synthesis and online execution. We demonstrate, in simulation, our framework's capabilities to discover missing locomotion skills and react promptly in safety-critical environments, such as scattered stepping stones and rebars.

==> journal_tex/abstract.tex <==
\begin{abstract}
This study proposes a two-stage, integrated planning framework for quadrupedal locomotion over dynamically changing, unforeseen terrains.
Existing footstep planning approaches either rely heavily on heuristics, compromising safety and reliability, or directly solve a holistic optimization, suffering from expensive computation as terrain features become complex.
To address this challenge, our approach integrates reactive synthesis and Mixed-Integer Convex Program (MICP) to leverage the strength of both approaches. Specifically, we employ reactive synthesis to provide formal safety guarantees at the abstraction level and MICP to ensure footstep planning with physical feasibility for each symbolic transition.
To handle unrealizable specifications due to limited feasible symbolic transitions, we leverage a symbolic repair process to identify dynamically feasible missing skills in both offline and online phases. 
During the online execution phase, we re-run the MICP using real-world terrain data to bridge the gap between offline synthesis and online execution, along with online symbolic repair to handle unforeseen terrains.
Extensive simulations demonstrate the efficacy of our framework in discovering missing locomotion skills and enabling prompt reactions to safety-critical environments, such as scattered stepping stones and rebars.
\end{abstract}

==> journal_tex/approach.tex <==
\section{Approach Summary}
To tackle the above problems, our planning framework consists of two main modules: 
offline synthesis (Sec.~\ref{sec:reactive_gait_synthesis}) 
and
online execution (Sec.~\ref{sec:online_execution}), as shown in Fig.~\ref{fig:system_diagram}.
% a MICP planner (Sec.~\ref{sec:motion_primitive}),
% and a tracking controller (Sec.~\ref{sec:tracking_control}). 

The offline synthesis module generates a strategy that moves the robot to a set of predefined goal waypoints among possible terrain polygons,
utilizing a MICP planner to obtain feasible robot skills corresponding to the symbolic transition.
% If the skills are not enough to generate a strategy for the robot to reach any goal waypoint over any possible terrain states, we leverage symbolic repair to generate new skills and utilize the gait-free MICP planner to check the feasibility of the suggestions.
Instead of considering predefined goals and terrains as done during offline, the online execution module
takes in an online local waypoint
produced by a global navigation planner,
along with the online segmented terrain polygons \cite{miki2022elevation}.
% a global navigation planner provides a series of local goal waypoints,
% and a perception module 
%
% supplies the segmented terrain information.
It then executes the strategy to navigate the robot toward the goal waypoint, 
utilizing the same MICP planner but with online terrain segments,
and leverages online repair 
% (Sec.~\ref{sec:online_repair}) 
to handle unexpected terrain configurations.

==> journal_tex/conclusion.tex <==
\section{conclusion}
In this work, we presented an integrated planning framework for terrain-adaptive locomotion that combines reactive synthesis with MICP, enabling safe and reactive responses in dynamically changing environments. 
To address unrealizable specifications arising from limited motion primitives, we introduced a symbolic repair approach that incorporates dynamic feasibility checks, automatically identifying missing transitions necessary for navigating adversarial terrains. In the online execution phase, we tackled the disparity between offline synthesis and real-world conditions by using an online MICP solver and an online symbolic repair process based on real-world terrain data. New terrain conditions encountered during execution. 
Our approach not only enhances motion feasibility and safety but also provides a scalable solution for legged robots maneuvering in complex and safety-critical environments. Future work will involve extensive hardware testing to validate the proposed framework in real-world scenarios. Additionally, we plan to explore specifications of greater complexity to further test the algorithmic scalability.

==> journal_tex/discussion.tex <==
\section{Discussion}
\subsection{Generalization to More Types of Terrain}
Currently, it requires expert knowledge on categorizing the terrains.

\subsection{Perception Module}

\subsection{Optimality}

==> journal_tex/hardware.tex <==
\section{Hardware Demonstrations}
We demonstrate the entire framework on both unstructured and rebar scenarios.
\subsection{Unstructured Terrain}

\subsection{Rebar}

==> journal_tex/introduction.tex <==
\section{Introduction}
% New outline:

% 1. The primary motivation for using reactive synthesis in terrain-adaptive locomotion lies in its contributions to safety and computational efficiency. First, reactive synthesis provides a formal method to ensure safety by systematically considering possible interactions between the robot and surrounding adversarial terrains. Second, it abstracts complex and rich features of the environment, enabling faster computation compared to traditional methods that directly reason about the intricate relationship between the environment and robot dynamics.

% 2. Symbolic repair is crucial for guiding the search for necessary gait configurations traversing adversial terrains. One reason is that it reduces the effort needed to identify all essential skills required for different terrains. Additionally, symbolic repair facilitates the accumulation of experience. As repairs are conducted, the robot identifies and stores necessary skills, progressively enhancing its capabilities as it encounters a wider variety of terrains.

% 3. During the online phase, we address the gap between discrete abstraction and real-world information for both the robot and its environment. This is achieved by solving the MICP in real-time using up-to-date robot and terrain data. Online repair also utilizes real-time terrain information to handle previously unseen environments that were not encountered during offline synthesis. Unlike learning-based approaches, which may struggle with out-of-distribution terrains, our method remains adaptable to new conditions.

Terrain-adaptive locomotion is crucial for enhancing the traversing capabilities of legged robots and advancing beyond blind walking \cite{di2018dynamic,kim2019highly, zhou2022momentum}. Existing approaches often use heuristics \cite{fankhauser2018robust,jenelten2020perceptive,agrawal2022vision,grandia2023perceptive, asselmeier2024hierarchical} to simplify foot placement selection given a nominal reference trajectory. However, formal guarantees on locomotion safety, considering the robot's physical capabilities, are rarely explored—despite their importance in safety-critical scenarios like hazardous debris and construction sites. Moreover, complex features of surrounding terrains significantly increase the computational burden for optimization-based methods, such as mixed-integer program (MIP) \cite{valenzuela2016mixed,shirai2022simultaneous,jiang2023locomotion}, which directly address the interplay between terrain segments and robot kinematics and dynamics. Other MIP-based methods rely on simplifications to enhance speed, \textit{e.g.}, assuming predetermined contact sequences and timing \cite{deits2014footstep,ponton2016convex,ding2020kinodynamic,tonneau2020sl1m,risbourg2022real,acosta2023bipedal} or fixing the number of footsteps \cite{aceituno2017simultaneous}, but still face challenges in scaling up with the number of terrain segments.

Motivated by this fact, our study aims to combine formal control methods, \textit{i.e.}, linear temporal logic (LTL)-based reactive synthesis \cite{bloem2012synthesis}, with MIP-based approaches, to safely and promptly react to dynamically changing environments. Continuous robot states and local environments are abstracted into symbolic states to systematically study high-level interactions between the robot and surrounding challenging terrains such as obstacles and large gaps exceeding the robot's physical limit. Then, a Mixed-Integer Convex Program (MICP) is solved to provide a physical feasibility certificate and continuous trajectories for each symbolic transition. This integrated framework not only bridges the gap between high-level abstraction and low-level physical capabilities but also alleviates the computational burden of MICP through symbolic-level guidance, focusing on a nominal desired direction and specific regions to explore.
% focusing on a nominal desired moving direction and limiting the number of regions to explore. 
The proposed approach focuses on assuring safety and goal completeness in the local environment, thus is flexible in that it can be used to follow commands from a global/higher-level path planner \cite{wermelinger2016navigation, fernbach2017kinodynamic,norby2020fast,chignoli2022rapid,liao2023walking,feng2023gpf} or from a user, and can incorporate additional locomotion behavior as needed.

Enabling complex reasoning about physical interaction with a terrain-feature-rich environment requires an accurate abstraction of the robot states or terrain. For instance, multiple types of terrains might be defined based on the terrain height, orientation, and size, etc. However, this induces a scalability challenge, particularly when evaluating numerous symbolic transitions for underactuated, hybrid systems such as legged robots. Rather than solving for abundant feasible transitions \cite{bhatia2010sampling,liu2013synthesis,maly2013iterative,gu2022reactive} for each terrain combination (moving from one terrain type to another), it is more computationally efficient to utilize existing motion primitives such as a fixed set of gait configurations, and ensure traversability among a limited set of terrains selected by prior knowledge or experience. In addition, merely deploying the existing proven feasible motion primitives provides another layer of safety.
However, missing enough transition capabilities
often leads to \textit{unrealizable specifications}. Therefore, it is essential to develop a method that automatically identifies physically feasible symbolic transitions necessary for legged robots to maneuver in challenging environments. In this work, we adopt a symbolic repair approach based on \cite{pacheck2022physically}, incorporating dynamic feasibility checks, to design missing yet necessary motion primitives for our terrain-adaptive locomotion problem.

During online execution of a synthesized high-level transition strategy, two critical issues may arise, potentially leading to execution failures. First, discrepancies between offline-checked terrain and real-world one are often inevitable, and can lead to a mismatch between the desired symbolic transition and what is physically possible. Second, newly encountered terrains may also make the symbolic specifications unrealizable, as they were not accounted for during offline synthesis. %Existing efforts in the LTL synthesis literature address unexpected environmental changes and robot action failures mainly at the specification level \cite{livingston2012backtracking,ehlers2014resilience,guo2013revising,li2021reactive,zhou2022reactive,cao2022leveraging,meng2024automated}. Studies that consider both robot and environmental mismatches at symbolic and physical levels remain largely underexplored, yet become increasingly crucial for safety-critical, terrain-adaptive locomotion. 

In this work, we solve an MICP online while executing the synthesized transition strategy, using real-world terrain data to ensure motion feasibility and fidelity. More importantly, an online symbolic repair is performed, similar to the offline repair, to identify possible transitions based on the new terrain and updated feasibility provided by the online MICP, allowing the robot to explore previously unseen terrains.
% for progressive generalization to a wider range of terrains.

The primary contributions of this paper are as follows:
\begin{itemize}
    \item We propose an integrated planning framework for terrain-adaptive locomotion by combining reactive synthesis with MICP. This framework generates motion primitives, a computationally expensive process, based on the actual needs of the robot, by leveraging symbolic search over an abstraction to limit the number of required motion primitives.
    %\item To address unrealizable specifications due to limited predefined motion primitives, we introduce a symbolic repair approach that incorporates dynamic feasibility checks, and automatically identifies the missing but necessary transitions for legged robots to effectively navigate adversarial terrains.
    \item During online execution, we address the disparity between offline synthesis and real-world terrain conditions at both physical and symbolic levels. Our approach leverages an online MICP solver along with an online symbolic repair process to account for real-world terrain discrepancies and newly encountered conditions, enhancing motion feasibility and safety during execution.
    % \item The entire framework is implemented in an online manner and validated through both simulation and hardware experiments. To the best of our knowledge, this is the first real-time local planner that determines both gait and foothold with a safety guarantee.
\end{itemize}

==> journal_tex/offline_synthesis.tex <==
\section{Offline Synthesis}\label{sec:reactive_gait_synthesis}
% \section{Reactive Synthesis for Locomotion}\label{sec:reactive_gait_synthesis}
% As illustrated in Fig.~\ref{fig:combined_offline_online}, 
The offline synthesis module 
% $\inpstateterrainposs \subseteq 2^\inpterrain$,
% and 
generates a strategy 
that enables the robot
to reach desired goal waypoints over all predefined terrain states.
%
As shown in Fig.~\ref{fig:combined_offline_online}(a),
this module takes in
a set of request goals and
a set of possible terrain states from prior knowledge of the workspace. In addition, a set of locomotion gaits is also provided by the user. After discretizing the local environment and characterizing the terrains in Sec.~\ref{sec:preliminaries_abstraction}, we first solve a gait-fixed MICP problem to determine the feasibility of each potential skill given the locomotion gaits
(Sec.~\ref{sec:motion_primitive}), and then encode all feasible transitions as skills in a specification
(Sec.~\ref{sec:spec_gen}).
If the specification is realizable, we generate a strategy for online execution.
Otherwise, we leverage a repair process to suggest new robot skills, utilize the gait-free MICP planner to check the feasibility of the suggested skills, and eventually make the specification realizable
(Sec.~\ref{sec:symbolic_repair}).


% The reactive synthesis process has two phases: offline synthesis and online execution. 
% We begin by introducing the essential specifications that define our terrain-adaptive locomotion problem. The objective is to construct a high-level robot gait and keyframe transition strategy by solving a two-player game between the gait planner and its possibly adversarial environment. The Linear Temporal Logic (LTL) specifications are designed by human experts, who provide logical rules that guide the planning process. It is nothworthy that the specification design is not unique and may vary according to expert input.

% Add a mapping function from the discrete state to the continuous state?

% \subsection{Motion Primitives to Robot Skills}\label{sec:motion_primitive}
\subsection{Locomotion Gait and Feasibility Checking via MICP}\label{sec:motion_primitive} 
We assume each locomotion gait comes with a contact sequence $\mathcal{G}$ and corresponding time durations $T$. Therefore, we define the locomotion gait as $L = \mathcal{M}(\mathcal{G}, T)$. Each skill is assumed to have a unique locomotion gait to determine how the robot moves at the continuous level. 
As shown in Fig.~\ref{fig:combined_offline_online}(a), since all the possible request goals $\inprequest$ and terrain states $\inpterrain$ are predefined during the offline phase, it is straightforward to first identify all the potential skills at the symbolic level that allow the robots to move freely in all possible local environments. In most examples shown in this paper, we assume the robot is only allowed to move horizontally and vertically by one cell and we show diagonal movements and heading angle change in Sec.~\ref{sec:extension}.
% Then, 
% we formulate a MICP problem that
% each MICP solve can 
% takes in 

Then the next critical step is to find whether there exists a locomotion gait for each skill to be physically feasible.
We leverage mixed-integer convex programming (MICP) to check the physical feasibility given a set of predefined locomotion gaits, and only use the feasible one as robot skills to synthesize robot strategies. The MICP problem takes in
the centroidal states $\inpcen$ from the precondition and postcondition of the skill as its initial and final conditions, which are located at the center of each abstracted cell. A set of homogeneous, predefined terrain polygons are considered in the MICP as steppable regions corresponding to the terrain states $\inpterrain$ involved in the precondition. Lastly, the contact information $\mathcal{G}$ and $T$ is provided by the selected locomotion gait $L$. Fig.~\ref{fig:mip_go2} shows the maneuver of the quadruped robot Go2 after solving the MICP problem corresponding to skill $a_0$ in Example~\ref{example:1} with a one-second trotting locomotion gait. The generic MICP problem considered in this work can formulated as:
    \begin{subequations}\label{ocp:mip_general}
    \begin{alignat}{2}
        \nonumber &\underset{\vg \phi, \v H}{\min} && \sum_{i = 0}^{N-1} \hspace{2pt} C(\vg \phi[i], \vg \phi_{\text{ref}}[i])\\
        & \text{s.t. } && \vg \phi[0] = \vg \phi_{\text{init}} \\& && \vg \phi[N-1] = \vg \phi_{\text{final}} \\
     & &&  \vg \phi[i+1] = \mathcal{D}(\vg \phi[i]), \forall i \in \range{N} \\
        & && \v g(\vg \phi, \v H, i) = 0 \\
        & && \v h(\vg \phi, \v H, i) \geq 0
    \end{alignat}
\end{subequations}
where the decision variables $\vg \phi$ denote the continuous variables and $\v H$ indicate the binary variables across the entire $N$ timesteps. For any natural number $n \in \naturals$, we denote the set $\{0, \dots, n-1\}$ as $\range{n}$. The general equality constraints $\v g(\cdot)$ and inequality constraints $\v h(\cdot)$ are incorporated and activated at certain time stamp $i$. The cost function depends on both the continuous variables $\vg \phi$ and a reference trajectory $\vg \phi_{\text{ref}}$.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{mip_go2.pdf}
    \caption{Demonstration of decision variables and polygons when solving MICP for skill $a_0$ in Example~\ref{example:1} using a trotting locomotion gait.}
    \label{fig:mip_go2}
\end{figure}

The reference base position and angular trajectories are generated by linearly interpolating between the initial and final conditions. For scenarios with significant elevation changes, such as jumping onto higher terrain, an additional middle keyframe is introduced for the pitch angle to calculate the slope angle between the initial and final poses. The final reference pitch trajectory is then created by evenly interpolating between the initial, middle, and final poses. The reference EE trajectory relative to the base frame $^\mathcal{B} \v p_j^{\text{ref}}$ remains constant and moves in sync with the reference base trajectory.

Given a specific locomotion gait, we first introduce the gait-fixed MICP formulation:

\subsubsection{Continuous Decision Variables}
The continuous decision variables $\vg \phi$ include base position $\v r$, velocity $\dot{\v r}$, acceleration $\ddot{\v r}$, orientation $\vg \theta$ parameterized by Euler angle and its first and second-order derivatives $\dot{\vg \theta},\ddot{\vg \theta}$, individual end-effector (EE) position $\v p_j$, velocity $\dot{\v p}_j$, and acceleration $\ddot{\v p}_j$, and individual contact force $\v f_j$ for the foot $j$ with $j\in\range{n_f}$, where $n_f=4$ denotes the index of feet. The compact form can be expressed as:
\begin{equation}
    \vg \phi^{\top} = [\v r^\top, \dot{\v r}^\top, \ddot{\v r}^\top, \vg \theta^\top, \dot{\vg \theta}^\top, \ddot{\vg \theta}^\top, \v p_j^\top, \dot{\v p}_j^\top, \ddot{\v p}_j^\top, \v f_j^\top]^\top
\end{equation}

\subsubsection{System Dynamics}
We encode the system dynamics as a simplified single rigid body in Eq.~(\ref{eq:dynamics}),
using a double integrator to replace the original Euler equation to keep the dynamics constraint convex. The whole system is discretized through Backward Euler integration with $\Delta t$ between each time step.
\begin{equation}
        \label{eq:dynamics}
        \begin{bmatrix} \v r[i+1]\\\
        \dot{\v r}[i+1]\\\
        m \ddot{\v r}[i]\\\
        \vg \theta[i+1]\\
        \dot{\vg \theta}[i+1]
        \end{bmatrix}= \begin{bmatrix}
        \v r[i] + \Delta t \cdot \dot{\v r}[i+1]\\
        \dot {\v r}[i] + \Delta t \cdot \ddot{\v r}[i+1]\\
        \sum\nolimits_{j} \v f_j[i] + m \v g \\
	    % \sum\nolimits_j (\v{p}_j[i] - \v r[i]) \times \v f_j[i] \\
            \vg \theta[i] + \Delta t \cdot \dot{\vg \theta}[i+1]\\
            \dot{\vg \theta}[i] + \Delta t \cdot \ddot{\vg \theta}[i+1]
	    \end{bmatrix}
\end{equation}
where $m$ is the robot mass and $g$ is the gravity term.

\subsubsection{Cost Function}
The cost function consists of tracking costs and regularization terms governed by diagonal matrices $\v Q$ and $\v R$. 
\begin{equation}
    \v C = \delta \vg \phi_Q[i]^T\mathbf{Q}\hspace{2pt}\delta \vg \phi_Q[i] + \vg \phi_R[i]^{T}\mathbf{R}\vg \phi_R[i]
\end{equation}
where $\delta \vg \phi_Q$ and $\vg \phi_R$ are defined as:
\begin{equation}
    \delta \vg \phi_Q = \begin{bmatrix}
        \v r - \v r_{\text{ref}}\\
        \vg \theta - \vg \theta_{\text{ref}}\\
        \v p_j - \v p_{j}^{\text{ref}}
    \end{bmatrix}, \vg \phi_R = \begin{bmatrix}
        \ddot{\v r}\\
        \ddot{\vg \theta}\\
        \ddot{\v p}_j\\
        \v f_j
    \end{bmatrix}
\end{equation}

Tracking costs include deviation from the desired base and foot EE trajectories. The regularization term includes minimizing the base acceleration, Euler angle acceleration, EE acceleration, and contact forces to encourage motion smoothness. The weights for the tracking terms are defined in Table~\ref{tab:cost_weights}.
\begin{table}[t]
    \caption{Tracking Cost Weights}
    \centering
     \begin{tabular}{c | c}
         \hline
         Cost Term & Weights\\\hline
         $\v r - \v r_{\text{ref}}$ & (1000.0, 1000.0, 1000.0)\\
         $\vg \theta - \vg \theta_{\text{ref}}$ & (1000.0, 1000.0, 1000.0)\\
         $\v p_j - \v p_{j}^{\text{ref}}$ & (1000.0, 1000.0, 1000.0)\\
         $\ddot{\v r}$ & (10.0, 10.0, 10.0)\\
         $\ddot{\vg \theta}$ & (10.0, 10.0, 10.0)\\
         $\ddot{\v p}_j$ & (0.5, 0.5, 0.5)\\
         $\v f_j$ & (0.1, 0.1, 0.1)\\
         \hline
    \end{tabular}
    \label{tab:cost_weights}
\end{table}



% \qm{plz also explain $N, n_f, n_s,$ and $R$}

% \subsubsection{Collision Avoidance}

\subsubsection{Safe Region Constraint}
To incorporate safe region constraints for selecting proper footholds, we introduce binary variables $\v H_{r,k,j}$, with $r$, $k$, and $j$ expressing the $r^{\rm th}$ convex region, $k^{\rm th}$ footstep, and $j^{\rm th}$ foot and $r\in\range{R}, k\in\range{n_s}$. One footstep is defined as a full swing phase for a foot. We use $n_s$ and $R$ to represent the number of footsteps specified by the gait configuration and the number of convex terrain polygons to be considered. For example,  Fig.~\ref{fig:mip_go2} shows a case with eight polygons.
Eqs.~(\ref{eq:safe_region}) - (\ref{eq:safe_region_eq}) restrict
the robot's EE to stay within one of the convex polygons described by an inequality ($\v A_r$ and $\v b_r$) and an equality ($\v A_{\text{eq},r}$ and $\v b_{\text{eq},r}$) constraint when the corresponding binary variable $H_{r,k,j}$ is True. We use $\mathcal{C}_{k,j}$ to denote the set of time steps indicating stance after the $k^{\rm th}$ footstep for the $j^{\rm th}$ foot and the safe region constraint only applies to the first stance time step represented as $\mathcal{C}_{k,j}[0]$. Note that, during the offline phase, the terrain polygons are homogeneous and predefined.
\begin{align}
\nonumber
&\forall r \in [R], k \in [n_s], j \in [n_f]\\
    \label{eq:safe_region} &\v H_{r,k,j} \Rightarrow \v A_r \v p_j[i] \leq \v b_r, \forall i \in \mathcal{C}_{k,j}[0]
        \\\label{eq:safe_region_eq} & \hspace{1.5cm} \v A_{\text{eq},r} \v p_j[i] = \v b_{\text{eq},r}, \forall i \in \mathcal{C}_{k,j}[0]
        \\&\sum_{r=0}^{R-1}\v H_{r,k,j} = 1
        \\&\v H_{r,k,j} \in \{0, 1\}
\end{align}

\subsubsection{Frictional and Contact Constraints}
Frictional constraints are defined in Eqs.~(\ref{eq:force_non_zero}) - (\ref{eq:force_friction_cone}), with $\v n_r$ and $\mathcal{F}_r$ as the normal vector and friction cone of the $r^{\rm th}$ convex region corresponding to the x and y dimensions of the EE position $\v p^{xy}_j$. Contact constraints in Eqs.~(\ref{eq:ee_velocity_zero}) - (\ref{eq:force_zero}) forces the EE velocity to be zero during stance phase and the contact force to be zero during the non-contact phase. $\mathcal{C}_{j}$ represents the set of all time steps indicating stance for the $j^{\rm th}$ foot.
\begin{align}
    \nonumber &\forall r \in [R], k \in [n_s], j \in [n_f]\\\label{eq:force_non_zero}
    &\v H_{r,k,j} \ \  \Rightarrow \ \ \v f_j[i] \cdot \v n_r(\v p_j^{xy}[i]) \ge 0, \ \forall i \in \mathcal{C}_{k,j}\\
    \label{eq:force_friction_cone}
        & \hspace{1.95cm} \v f_j[i] \in \mathcal{F}_r(\mu, \v n_r, \v p_j^{xy}[i]), \ \forall i \in \mathcal{C}_{k,j}
         \\\label{eq:ee_velocity_zero}
            &\dot{\v p}_j[i]=0, \ \forall i \in \mathcal{C}_j
        \\\label{eq:force_zero}
         &\v f_j[i] = 0, \ \forall i \notin \mathcal{C}_j
\end{align}
%
where $\mu$ denotes the friction coefficient.

\subsubsection{Actuation Constraint}
Since the joint angles are omitted in the single rigid body model, we use a fixed Jacobian $\v J_j(\v q_j^{\text{ref}})$ at a nominal joint pose $\v q_j^{\text{ref}}$ for each leg to approximately consider the torque limit constraint in Eq.~(\ref{eq:max_torque}). In addition, since the translational and angular motions are decoupled, another actuation constraint on the angular acceleration is also added in Eq.~(\ref{eq:max_acc}).
\begin{align}
\nonumber & \forall i \in [N], j \in [n_f] \\
    \label{eq:max_torque}
& \v J_j(\v q_j^{\text{ref}})^{\top} \v f_j[i] \leq \vg \tau_{\rm max}\\\label{eq:max_acc}
& \v I \ddot{\vg \theta}[i] \leq \vg \tau_{\rm max}^{\prime}
\end{align}
where $\vg \tau_{\rm max}$ is the joint torque limit, $\vg \tau_{\rm max}^{\prime}$ is the torque limit applied on the base, and $\v I$ is the moment of inertia for the approximated single rigid body.

\subsubsection{Kinematics Constraint}
Lastly, the kinematics constraint in Eq.~(\ref{eq:rom}) strictly limits the possible EE movements to assure safety.
% Fig.~\ref{fig:mip_a1} shows the essential decision variables optimized in \ref{ocp:mip_general}. 
Due to the convex nature of this MICP, we can determine the feasibility of a possible symbolic transition by checking if the optimal solution exists.
\begin{equation}
    \label{eq:rom}
    \v p_j[i] \in \mathcal{R}_j(^\mathcal{B} \v p_j^{\text{ref}}, \v r[i],\vg \theta_{\text{ref}}, \v p_j^{\text{max}}), \forall i \in [N], j \in [n_f]
\end{equation}
where $\mathcal{R}_j$ is defined as a 3D box constraint around a nominal foot EE position based on the base position and orientation, and constrained by a maximum deviation $\v p_j^{\text{max}}$. Note that the reference orientation $\vg \theta_{\text{ref}}$ is used to avoid nonlinear constraint keep the problem convex.

%%%% Fig4. System overview %%%%
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{combined_offline_online_v2.pdf}
    \caption{System overview for offline synthesis and online execution modules. During the offline synthesis (pink solid arrows), an initial set of motion primitives is given and symbolic skills are iteratively generated by solving MICP. When the task specifications are unrealizable, a symbolic repair is triggered to seek missing skills. During the online execution (black solid arrows), MICP is solved again taking online terrain segments and the symbolic state only advances when a solution is found. Online repair is triggered (blue solid arrows) when a solving failure or an unseen terrain is detected. 
    % both abstracted and real-world terrain information is fed into the automaton.
    }
    \label{fig:combined_offline_online}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{GR(1) Specifications given Robot Skills}\label{sec:spec_gen}
\subsection{Task Specification Encoding}\label{sec:spec_gen}

After acquiring a set of feasible robot skills, 
we encode the skills into the specification $\spec$ 
as part of the environment safety assumptions $\envsafety$ 
and system safety guarantees $\syssafety$.
%
% We divide the safety assumptions $\envsafety$ into mutable assumptions $\envsafetynothard$,
% which describe the postconditions of the skills,
% and hard assumptions $\envsafetyhard$ that cannot be modified, 
% i.e.
% $\envsafety = \envsafetynothard \land \envsafetyhard$.
% Similarly, we divide the safety guarantees $\syssafety$ into mutable guarantees $\syssafetynothard$,
% which represent the preconditions of the skills,
% and hard guarantees $\syssafetyhard$ that cannot be modified
% ($\syssafety = \syssafetynothard \land \syssafetyhard$).
%
% To translate from states to formulas, 
We define a function $\formplain$ that takes as input
two subsets $\statevar, \statevar' \subseteq \ap$,
where $\statevar \subseteq \statevar'$,
and generates a Boolean formula
$\form{\statevar'}{\statevar} \coloneqq \bigwedge_{\var\in\statevar}\var \land \bigwedge_{\var \in \statevar'\setminus\statevar} \neg\var$.
For any subset $\statevar \subseteq \ap$,
we use $\bigcirc\statevar$ to denote the set $\{\bigcirc \pi \mid \pi \in \statevar\}$.

% We encode the postconditions of the skills into the environment safety assumptions $\envsafety$ of the specification $\spec$.



% each skill $\texttt{skill} \in \mathcal{A}$ comes with a precondition $\sum_{\texttt{skill}}^{\rm{pre}} \in 2^{\mathcal{I}_G}$ and a postcondition $\sum_{\texttt{skill}}^{\rm{post}} \in 2^{\mathcal{I}_G}$ similar to \cite{pacheck2022physically}. In Fig.~\ref{fig:preliminary_nine_squares}(b) and (c), it shows a skill $\texttt{skill0}$ with precondition $\sum_{\texttt{skill0}}^{\rm{pre}} = \{(x=1,y=2,\rm cT = \rm Flat, \rm rT = \rm High)\}$ and postcondition $\sum_{\texttt{skill0}}^{\rm{post}} = \{(x=2,y=2)\}$. The skills are encoded in the GR(1) formula as part of $\phi^\textrm{t}_\textrm{e}$ and $\phi^\textrm{t}_\textrm{s}$, 
% which can be further divided into $\phi^{\textrm{t}}_{\textrm{e}} = \phi^{\textrm{t, mutable}}_{\textrm{e}} \wedge \phi^{\textrm{t, hard}}_{\textrm{e}}$ and $\phi^{\textrm{t}}_{\textrm{s}} = \phi^{\textrm{t, mutable}}_{\textrm{s}} \wedge \phi^{\textrm{t, hard}}_{\textrm{s}}$. $\phi^{\textrm{t, mutable}}_{\textrm{e}}$ and $\phi^{\textrm{t, mutable}}_{\textrm{s}}$ capture the postconditions and preconditions that the repair process might modify, respectively. $\phi^{\textrm{t, hard}}_{\textrm{e}}$ and $\phi^{\textrm{t, hard}}_{\textrm{s}}$ encode the hard constraints specified by the user remain unchanged and always hold.   

% \subsubsection{Postconditions}
The skill assumptions $\envsafetynothard$ encode the postconditions of the skills. 
% As shown in Eq.~\ref{eq:env_trans}, 
The assumptions ensure that after the skill execution, 
at least one postcondition of the skill must hold:
% s in the next timestep:

\begin{equation}\label{eq:env_trans}
\begin{aligned}
    \envsafetynothard \coloneqq \bigwedge_{\skill \in \mathcal{O}} \big( \skill 
    % \land 
    % \form{\inpcen\cup\inpterrain}{\skillpre} \\ 
    \to
    \bigvee_{\statevar\in\skillpost} \form{\bigcirc\inpcen}{\bigcirc\statevar} \big)
    % \bigvee_{\sigma_\textrm{pre} \in \sum_{\texttt{skill}}^\textrm{pre}} \varphi_{\sigma_{\textrm{pre}}}) \rightarrow \\
    % &\bigcirc \bigvee_{\sigma_\textrm{post} \in \sum_{\texttt{skill}}^\textrm{post}} \varphi_{\sigma_\textrm{post}}\bigg)
\end{aligned}
\end{equation}
%
In Example~\ref{fig:preliminary_nine_squares},
% $\skillprecustom{\skillcustom{0}}$,
the postcondition of skill $\skillcustom{0}$
is defined as:
% encoded asin Eq.~\ref{eq:skill_0_post}:
% Therefore, as an example, the postcondition specification for $\texttt{skill0}$ is defined as:
\begin{equation}\label{eq:skill_0_post}
\begin{aligned}
     \square (\skillcustom{0} 
     % \land x_1 \land y_1 \land \tvar{x_1}{y_0} \land \tvar{x_1}{y_1} \land \tvar{x_1}{y_2}
     % \land \bigwedge_{\var\in\inpcen\cup\inpterrain\setminus\skillprecustom{\skillcustom{0}}} \neg \var \\
    \to &\bigcirc x_0 \land \bigcirc y_1 \land \neg \dots)
    % &\neg \bigcirc x_1 \land 
    % \neg \bigcirc x_2 \land 
    % \neg \bigcirc y_0 \land 
    % \neg \bigcirc y_2 \big)
     % \bigwedge_{\var\in\inpcen\setminus\skillpostcustom{\skillcustom{0}}} \neg \bigcirc \var \big)
     % x=1 \wedge y=2 \wedge \rm cT = \rm Flat \wedge \rm rT = \rm High \big) \rightarrow \\
     % &\bigcirc \big(x=2 \wedge y=2 \big) \big)
\end{aligned}
\end{equation}
where we omit the centroidal inputs that are False.

% \subsubsection{Preconditions}
The skill guarantees $\syssafetynothard$ encode the preconditions of the skills.
The guarantees impose restrictions on when a skill can be executed.
% As shown in Eq.~\ref{eq:sys_trans},
The guarantees only allow the robot to execute a skill 
if one of the skill's preconditions holds:
% The preconditions encode constraints in $\varphi_{\textrm s}^{\textrm{t}, \textrm{mutable}}$. It restricts the conditions that a specific skill can be chosen. Therefore, it allows the overall system to choose a skill only when a precondition is satisfied, but does not require the system to do so. 

\begin{equation}\label{eq:sys_trans}
\begin{aligned}
    \syssafetynothard \coloneqq 
    \bigwedge_{\skill \in \mathcal{O}} \bigg(
    \neg \big(
    \bigvee_{\statevar\in\skillprecustom{\skill}}
    \form{\bigcirc\inpcen\cup\bigcirc\inpterrain}{\bigcirc\statevar}
    \big)
    % \\
    % \form{\bigcirc(\inpcen\cup\inpterrain)}{\bigcirc\skillprecustom{\skill}}\\
    \to \neg \bigcirc \skill
    \bigg)
    % \\
    % \varphi_{\textrm s}^{\textrm{t}, \textrm{mutable}} = \bigwedge_{\pi_{\texttt{skill}} \in \mathcal{O}} \bigg( & \neg (\bigcirc \bigvee_{\sigma_\textrm{pre} \in \sum_{\texttt{skill}}^\textrm{pre}} \varphi_{\sigma_{\textrm{pre}}}) \rightarrow 
    % &\neg \bigcirc \pi_{\texttt{skill}}\bigg)
\end{aligned}
\end{equation}
%
In Example~\ref{example:1}, the precondition of skill $\skillcustom{0}$ is defined as:
\begin{equation}
\begin{aligned}
     \square \big( \neg 
     (
     \bigcirc x_1 \land 
     \bigcirc y_1 \land 
     \bigcirc \tvar{x_1}{y_0} \land 
     \bigcirc \tvar{x_1}{y_1} \land 
     \bigcirc \tvar{x_1}{y_2}\land \\
     \neg \dots)
     % \neg \bigcirc x_0 \land
     % \neg \bigcirc x_2 \land
     % \neg \bigcirc y_0 \land
     % \neg \bigcirc y_2 \land \\
     % \bigwedge_{i\in\{0,2\}, j\in\{0,1,2\}}
     % \neg \bigcirc \tvar{x_i}{y_j}\big)
     % \bigwedge_{\var\in\inpcen\cup\inpterrain\setminus\skillprecustom{\skillcustom{0}}} \neg \bigcirc \var
     % \big)
     % \\
     \to \neg \bigcirc \skillcustom{0} \big)
     % \\
     % (\bigcirc (x=1 \wedge y=2 \wedge \rm cT = \rm Flat \wedge \rm rT = \rm High)) \rightarrow \\
     % \neg \bigcirc \pi_\texttt{skill0}\big)
\end{aligned}
\end{equation}
where we omit the centroidal and terrain inputs that are False.
% include the keyframe transition action $\mathcal{K}$ and gait primitives $\mathcal{G}$. We further divide $\mathcal{G}$ into $\mathcal{G} = \{\rm{gaitType}, \rm{gaitSpeed}\}$. We incorporate extra input propositions $\mathcal{E}$ to represent the terrain information, which shows up in the preconditions as well.
% \subsubsection{Hard Constraints}\label{sec:hard_constraints}

The hard constraints ($\envsafetyhard$, $\syssafetyhard$) are constraints that a repair cannot modify 
(see Sec.~\ref{sec:symbolic_repair}).
To strictly guarantee $\syssafetyhard$,
we only allow the robot to execute one skill at a time:
    $\square\big(\neg (\bigcirc\skill \land \bigcirc\skill')\big)$, for any two different skills $\skill, \skill' \in \out$. Given that, 
    %such that $\skill \neq \skill'$.
we encode the following hard assumptions $\envsafetyhard$:
% as hard constraints in $\envsafetyhard$ and $\syssafetyhard$:
% The hard assumptions $\envsafetyhard$ states that
\begin{enumerate}[label=\arabic*),ref=\arabic*]
    \item The uncontrollable terrain and request inputs 
    % $\inpterrain \cup \inprequest$
    % which include the terrain and request inputs ($\inpuser = \inpterrain\cup\inprequest$), 
    cannot change during execution:
    % $\forall \var \in \inpuser$,
    $\square (\var \leftrightarrow \bigcirc \var)$,
    $\forall \var \in \inpterrain \cup \inprequest$.
    \item The centroidal inputs $\inpcen$ remain unchanged if no skill is executed: 
    $\square\big(\bigwedge_{\skill\in\out} \neg \skill \to \bigwedge_{\var\in\inpcen} (\var \leftrightarrow \bigcirc \var)\big)$.
    \item \label{assumption:poss_terrain}
    The terrain state must come from the set of possible terrain states $\inpstateterrainposs \subseteq 2^{\inpterrain}$ provided by the user:
    $\envterrain \coloneqq \square (
    \bigvee_{\statevar\in\inpstateterrainposs}
    \form{\inpterrain}{\statevar}
    )$.
\end{enumerate}

% Certain constraints also need to be incorporated as hard constraints. $\varphi_{\textrm e}^{\textrm{t}, \textrm{hard}}$ and $\varphi_{\textrm s}^{\textrm{t}, \textrm{hard}}$. For instance, specifications such as enforcing movements among adjacent grids are encoded as hard constraints. Other constraints such as the mutual exclusion of different skills are also added here. 

% For the nine-square example, we 

% Due to the space limit, we only highlight the specifications that build connections between the environment and the robot action. We construct the following specifications based on locomotion heuristics:

% Hard specifications. React to terrain abstraction. Mutual exclusion of each skill and each grounded state.



% \subsection{Offline Synthesis with Feasibility Check}
% Fig.~\ref{fig:combined_offline_online} illustrates the system overview for both offline synthesis and online execution. This section focuses on the offline synthesis process. Using prior knowledge provided by humans, we first define a set of motion primitives, such as a one-second trotting gait, and a set of potential terrains described at the symbolic level. Based on the abstracted robot and terrain states defined in Sec.\ref{sec:preliminaries_abstraction}, we iterate over the grid locations and solve the MICP to check if a solution exists when the desired goal is the adjacent grid. If a solution is found, the corresponding skill is added to the specification. Once the hard constraints and physically feasible skills are incorporated into the specification, we assess its realizability. If it is realizable, a strategy is generated for online execution. If not, an offline repair is introduced, as discussed in the next section.

\subsection{Symbolic Repair}\label{sec:symbolic_repair}
The specification $\spec$ generated in Sec.~\ref{sec:spec_gen} may be unrealizable
if the physical feasibility checking in Sec.~\ref{sec:motion_primitive} does not generate enough skills for the robot to reach all goal locations over all possible terrain combinations.
%
To adress this issue, we leverage the ideas in~\cite{pacheck2022physically} 
% to ensure that the generated specification $\spec$
% (Sec.~\ref{sec:spec_gen}) is realizable~\cite{pacheck2022physically}.
% The specification $\spec$ can be unrealizable if the physical feasibility checking (Sec.~\ref{sec:motion_primitive}) does not generate enough skills for the robot to traverse to all goal locations over all possible terrain combinations.
% The repair 
to
generate
new skill suggestions necessary for the robot to accomplish the task.
%over all possible terrain environments.
Different from~\cite{pacheck2022physically}, we assume that skills do not contain intermediate states,
and the skill preconditions
are over both the controllable centroidal inputs $\inpcen$ and uncontrollable terrain inputs $\inpterrain$, 
while the postconditions remain to contain 
controllable
centroidal inputs $\inpcen$ only.

% We extend repair to handle skills whose preconditions are over both the controllable centroidal inputs $\inpcen$ and terrain inputs $\inpterrain$ while the postconditions still only contain controllable inputs $\inpcen$.

For any subset $\statevar\subseteq \ap$, we say that $\statevar$ is a winning state
if the robot can guarantee to satisfy the task from $\statevar$
despite adversarial environment behaviors.
The repair process systematically expands the set of winning states until
it intersects with all liveness goals and contains all initial states.
To this end, the repair alternatively modifies the preconditions and postconditions of existing skills.
When modifying preconditions, the repair randomly selects a skill whose postcondition is winning, and modifies its precondition to a non-winning state, thus making the new precondition possible to win.
When modifying postconditions, the repair randomly selects a skill whose preconditions and postconditions are both non-winning, and modifies its postcondition to a winning state, thus making the original precondition possible to win.
%
Fig~\ref{fig:preliminary_nine_squares}c illustrates the use of repair in Example~\ref{example:1}. 
To create a skill that reaches the requested grid $(x_0, y_0)$, the
repair selects the skill transition that moves the robot from the grid $(x_1, y_0)$ to $(x_2, y_0)$,
and modifies the postcondition to reach $(x_0, y_0)$ instead. Finally, the suggested skills are sent to a gait reconfiguration module for feasibility checking. If any suggested skill is found infeasible, the symbolic transition is added as a hard constraint, and the repair process is repeated.

\subsection{Gait-Free MICP}
During the offline... We aim to implement the suggested skills by reconfiguring the contact sequence and timing to generate new locomotion gaits. This can be achieved by solving a gait-free version of MICP in Eq.~(\ref{ocp:mip_general}). The gait-free MICP retains all continuous decision variables and constraints from the gait-fixed MICP but modifies the contact state-dependent constraints, as the contact sequence and timing are no longer fixed. Instead of using $\v H_{r,k,j}$, we introduce a different set of binary variables $\v H_{r,m,j}$ for defining the contact state for each foot at each time step explicitly. $r$ and $j$ still represent the $r^{\rm th}$ convex region and $j^{\rm th}$ foot, respectively, while $m \in \range{M}$ denotes the $m^{\rm th}$ time step, evenly discretized with $\Delta t_m$ over the entire $M$ time steps. We use $\mathcal{O}_{m,m+1}$ to denote the set of continuous time steps that span from the $m^{\rm th}$ to the ${m+1}^{\rm th}$ binary time step. As a result, the following constraints are modified:
\subsubsection{Safe Region Constraint}
Different from Eq. The summation of the binary variables at $m^{\rm th}$ time step for the $j^{\rm th}$ foot is allowed to be zero to generate a swing phase.
\begin{align}
\nonumber &\forall r \in [R], m \in [M], j \in [n_f]\\    \label{eq:safe_region_2} &\v H_{r,m,j} \Rightarrow \v A_r \v p_j[i] \leq \v b_r, \forall i \in \mathcal{O}_{m,m+1}\\
    \label{eq:safe_region_2_eq} & \hspace{1.6cm} \v A_{\text{eq},r} \v p_j[i] = \v b_{\text{eq},r}, \forall i \in \mathcal{O}_{m,m+1}
        \\&\sum_{r=0}^{R-1}\v H_{r,m,j} \leq 1
        \\&\v H_{r,m,j} \in \{0, 1\}
\end{align}

\subsubsection{Frictional and Contact Constraints}
Different from the gait-fixed case, the activation of frictional and contact constraints is purely decided by the binary variables.
\begin{align}
    \nonumber & \forall r \in [R], m \in [M], j \in [n_f]\\    \label{eq:force_non_zero_2} & \v H_{r,m,j} \  \Rightarrow \ \v f_j[i] \cdot \v n_r(\v p_j^{xy}[i]) \ge 0, \forall i \in \mathcal{O}_{m,m+1}\\
    \label{eq:force_friction_cone_2}
        & \hspace{1.8cm} \v f_j[i] \in \mathcal{F}_r(\mu, \v n_r, \v p_j^{xy}[i]), \forall i \in \mathcal{O}_{m,m+1}
         \\\label{eq:ee_velocity_zero_2} &
        \sum_{r=0}^{R-1}\v H_{r,m,j} = 1 \ \Rightarrow \  \dot{\v p}_j[i]=0, \forall i \in \mathcal{O}_{m,m+1}
        \\\label{eq:force_zero_2} &
         \sum_{r=0}^{R-1}\v H_{r,m,j} = 0 \ \Rightarrow \ \v f_j[i] = 0, \forall i \in \mathcal{O}_{m,m+1}
\end{align}

Compared to gait-fixed MICP, gait-free MICP introduces more binary variables to determine contact states, resulting in longer computation times. As such, it is only triggered after performing symbolic repair.

==> journal_tex/online_execution.tex <==
\section{Online Execution}\label{sec:online_execution}
Due to the inevitable disparity between offline synthesis and real-world online terrain conditions, such as variations in terrain shape and position, additional efforts are required to bridge this gap and prevent potential execution failures. The online execution module takes in terrain states $\inpstateterrain \subseteq \inpterrain$ after abstracting the terrain polygons online, a request state $\inpstaterequest \subseteq \inprequest$,
and a strategy $\strategy$
from the offline synthesis module (Sec.~\ref{sec:reactive_gait_synthesis}).
This module then executes the strategy automaton $\strategy$
by solving a MICP problem online again with the actual perceived terrain polygons, potentially different from the ones abstracted offline, 
to generate a reference trajectory for each transition (Sect.~\ref{sec:automaton_online_evaluation}). This reference trajectory 
along with the corresponding contact information will be further tracked by a tracking controller in real time
(Sec.~\ref{sec:tracking_control}).
As shown by the blue lines in Fig.~\ref{fig:combined_offline_online}(c),
if the robot encounters an unseen terrain state, 
% is unexpected and thus not considered by the offline synthesis module,
we leverage online symbolic repair to create new skills that handle the unexpected terrain state and failure transition at runtime 
% $\inpstateterrain$ 
% and re-synthesize a strategy
(Sec.~\ref{sec:online_repair}).
After reaching the request state $\inpstaterequest$,
the robot resets the strategy with a new terrain state, request goal states,
and repeats the execution
until reaching the final goal state.






% During the online execution, we consider the mismatch between the abstracted and continuous information including both the robot and environmental states. 
% The online execution is divided into an online strategy execution process and a tracking control module.

\subsection{Strategy Automaton Execution and Online MICP Modifications}\label{sec:automaton_online_evaluation}
The red path in Fig.~\ref{fig:combined_offline_online}(c) represents the automaton online execution process. Before transitioning to the new symbolic state, an online gait-fixed MICP is solved according to the skill provided by the automaton. The automaton advances only if the MICP successfully finds a solution.
% Algorithm \ref{code:online_automaton} shows the complete steps of performing online evaluation. More specifically, we consider multiple.
% \subsubsection{Online MICP}
Slightly different from the gait-fixed MICP formulation during the offline phase, the online gait-fixed MICP is executed given accurate terrain information from a terrain segmentation module. 
For example, a skill transitioning from flat terrain to high terrain, as shown in Fig.~\ref{fig:online_micp}(a),  uses  predefined, homogeneous terrain polygons for feasibility check during offline synthesis. Given that, Fig.~\ref{fig:online_micp}(b) illustrates how the  terrain polygons detected online for the same skill may differ from the offline ones in both position and geometry.
% Since a strategy is already generated offline, the online MICP explicitly knows the chosen gait and the ideal initial and final robot states given by the robot and terrain abstraction.
In addition, the following modifications are highlighted when attempting to transition between two symbolic states in the automaton.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{online_micp.pdf}
    \caption{Demonstrations of (a) offline MICP for a skill transitioning from a flat terrain to a high terrain with predefined polygons; (b) online MICP for the same skill but with online terrain polygons.}
    \label{fig:online_micp}
\end{figure}


\subsubsection{Robot Pose Re-Targeting}
Since the final targeting condition significantly influences the reference trajectory and the feasibility of the MICP problem, we evaluate the final condition by solving a kinematic feasibility problem (a simplified MICP in Eq.~(\ref{ocp:mip_general})) before solving the online MICP. Compared with the gait-fixed MICP, the dynamics equation (\ref{eq:dynamics}) is replaced by enforcing the center of mass (CoM) to lie inside a convex support polygon with all feet in stance to ensure static stability. In addition, a hard constraint is added to ensure that the modified robot pose stays within a certain threshold compared with the original desired pose. The cost function is simplified to stay as close as possible to the original desired pose. The higher-order terms of body position, orientation, and end-effectors are excluded from the decision variables. All the other constraints not involving those higher-order terms remain the same. Once the kinematic feasibility problem is solved successfully, the online MICP is solved using the modified re-targeted final condition and reference trajectory.

\subsubsection{Collision Avoidance and Swing Foot Constraints}
Since the trajectory generated by the online gait-fixed MICP is directly sent to a tracking control module later, high-quality end-effector (EE) trajectories are crucial to ensure collision avoidance and sufficient swing foot clearance from the terrain. To achieve this, we first introduce more binary variables $\v H_{s,w,j}$ for defining the collision-free region selection for the $j^{\rm th}$ foot at each time step. Specifically, $s \in \range{S}$ represents the $s^{\rm th}$ convex collison-free region and $w \in \range{W}$ denotes the $w^{\rm th}$ time step, evenly discretized with $\Delta t_w$ over the entire $W$ time steps. Fig.~\ref{fig:online_micp}(b) demonstrates two collision-free regions.
\begin{align}
    \nonumber & \forall s \in [S], w \in [W], j \in [n_f]\\\label{eq:collision_avoidance} &\v H_{s,w,j} \Rightarrow \v A_s \v p_j[i] \leq \v b_s, \forall i \in \mathcal{C}_{w,w+1}
        \\&\sum_{s=0}^{S-1}\v H_{s,w,j} = 1
        \\&\v H_{s,w,j} \in \{0, 1\}
\end{align}
where $\mathcal{C}_{w,w+1}$ denotes the set of continuous time steps that span from the $w^{\rm th}$ to the ${w+1}^{\rm th}$ binary time step.

To enable larger swing foot clearance from the terrain in case of non-trivial tracking errors, we also add constraints to force the swing foot  height above a user-defined threshold $h_{\text{swing}}$, given the fixed contact timing.
% \begin{align}
%     &\v p_{j}^z[\text{mid}] \geq \v p_{j}^z[\text{start}] + h_{\text{swing}}\\
%     &\v p_{j}^z[\text{mid}] \geq \v p_{j}^z[\text{end}] + h_{\text{swing}}
% \end{align}
% where $\v p_{j}^z[\text{start}], \v p_{j}^z[\text{mid}], \v p_{j}^z[\text{end}]$ stand for the $j^{\rm th}$ EE positions in the z dimension at the starting, middle, and ending knot point of a swing phase, respectively. 

Note that the collision avoidance and swing foot constraints are also incorporated during the offline MICP as part of the feasibility checking rules. However, we highlight it here due to its critical impact on the tracking performance.

% \begin{algorithm}[h!]\label{code:strategy_execution}
%   \caption{Strategy Execution}
%   \SetAlgoLined
%   \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%   \PrintSemicolon
%    \Input{synthesized strategy $\mathcal{A}$, initial robot state $\v x_0$}
%    \Output{referenceTraj, gaitSequence}
%    \nl$\rm curNode$ = initializeNode($\v x_0$)\;
%     \nl\While{1}{
%         \texttt{// Roll out the automaton}\;
%         \nl\If{\rm previousWaypointReached}{
%         \texttt{// Check if local waypoint is changed}\;
%         \nl\If{\rm{!waypointPending} \& \textcolor{blue}{ \rm{localWaypointChanged}}}{
%             setNewWaypoint($\mathcal{X}_{\rm cen}^{\rm des}$, $\rm curNode$, $\mathcal{J}$)\;
%         }
%         \texttt{// Check if local terrain is changed}\;
%         \nl\If{\textcolor{blue}{\rm terrainStateChanged}}{
%             setUpdatedTerrain($\mathcal{E}$, $\rm curNode$, $\mathcal{J}$)\;
%         }
%         \texttt{// Find the next node and solve OCP}\;
%         \nl$\rm{nextNode}$ = findNextAllowableNode($\rm curNode$, $\mathcal{J}$)\;
%         \texttt{// Check goal pose feasibility}\;
%         \nl$\v x_{\rm init}$ = $\rm{referenceTraj}[-1]$\;
%         \nl($\rm goalFeasible$, $\v x_{\rm goal}$) = \textcolor{blue}{ solveInstantaneousOCP}($\rm nextNode$)\;
%         \nl\eIf{\rm goalFeasible}
%         {
%             \nl($\rm OCPsuccess$, $\rm traj$, $\rm gait$) = \textcolor{blue}{solveOCP($\rm curNode$, $\rm nextNode$)\;}}
%         {
%             \nl \textcolor{blue}{triggerReplan}\;
%         }
        
%         \nl\eIf{\rm OCPsuccess}{
%             \nl$\rm referenceTraj$ += $\rm traj$\;
%             \nl$\rm gaitSequence$ += $\rm gait$\;
%         }{
%             \nl \textcolor{blue}{triggerReplan}\;
%         }
%         \texttt{// Publish reference trajectory and gait}\;
%         \nl\If{$\mathcal{X}_{\rm cen} = \mathcal{X}_{\rm cen}^{\rm des}$}{
%             \nl publishReference($\rm referenceTraj$, $\rm gaitSequence$)\;
%             \nl clearReferenceTrajAndGait()\;
%             \nl \textcolor{blue}{requestReset}\;
%         }
%         \nl$\rm curNode$ = $\rm nextNode$\;
%         }
%         $\texttt{// Reset the current node}$\;
%         \nl\If{\rm resetRequested \& \rm{goalReached}} {
%             \nl$\rm curNode$ = findNodeAfterReset($\mathcal{E}$, $\rm curNode$, $\mathcal{J}$)\;
%         }
%     }
% \end{algorithm}

\subsection{Online Repair}\label{sec:online_repair}
During online execution, 
the robot may encounter unexpected terrain states
that the initial model of the workspace structure does not take into consideration.
We leverage an online repair tool~\cite{meng2024automated} 
to detect and recover from such unexpected terrain states.

The online repair tool first generates a monitor that detects violations of the environment assumptions $\envsafety$ during online execution.
%
Note that $\envsafety$ includes the assumption
$\envterrain = $ $
    \square (
    \bigvee_{\statevar\in\inpstateterrainposs}
    \form{\inpterrain}{\statevar})$,
which assumes that 
at any time, 
at least one terrain state from the set of possible terrain states $\inpstateterrainposs$ must hold
% the current terrain state $\inpstateterrain$
% must always come from
% $\inpstateterrainposs$, 
% the set of possible terrain states provided by the user
(see Sec.~\ref{sec:spec_gen}).
% Suppose the current terrain state $\inpstateterrain$ is not in $\inpstateterrainposs$, the set of possible terrain states provided by the user.
During online execution,
if the current terrain state $\inpstateterrain \not\in \inpstateterrainposs$,
the monitor detects that $\inpstateterrain$
violates the assumption $\envterrain$.
We then relax the violated assumption $\envterrain$ to admit the new terrain state $\inpstateterrain$,
replacing $\envterrain$ with 
$\square (
    \bigvee_{\statevar\in\inpstateterrainposs\cup\{\inpstateterrain\}}
    \form{\inpterrain}{\statevar})$.
After assumption relaxation,
the revised specification becomes unrealizable
as the robot lacks the required skills to handle the new terrain state $\inpstateterrain$.
We utilize symbolic repair 
(Sec.~\ref{sec:symbolic_repair})
to find a set of necessary skills for the new terrain state.






% the prior knowledge of the workspace structure does not take into account.
% \begin{enumerate}
%     \item Encounter unexpected terrain states during execution
%     \item Generate a monitor to check assumption violations
%     \item The monitor detects that the new terrain state violates the environment assumption which states that the current terrain state must belong to the set of possible terrain states.
%     \item we relax the assumption to include the new terrain state
%     \item we perform repair obtain new skills that can handle the new terrain state, and resume the execution
% \end{enumerate}


\section{Tracking Control}\label{sec:tracking_control}
The tracking control module adopts an MPC-Whole-Body-Control (WBC) hierarchy, ensuring precise end-effector (EE) and centroidal momentum tracking. To smoothly and efficiently execute the strategy considering the potential computational delay in solving MICP, a harmonic coordination module between the strategy automaton roll-out and the tracking module is designed (Sec.~\ref{sec:coordination}).

\subsection{Tracking Control Module}
\subsubsection{Nonlinear Model Predictive Control (NMPC)}\label{subsec:nmpc}
The NMPC  operates independently from the symbolic planning module, tracking reference trajectories generated by the online MICP using a more accurate dynamics model. In this work, the NMPC accounts for the robot's centroidal dynamics and kinematics, similar to approaches in \cite{dai2014whole,chignoli2021humanoid,sleiman2021unified}, presenting a more accurate model than the simplified angular dynamics in the MICP. An analytical inverse kinematics solution based on the MICP output provides the full joint state reference trajectory for the NMPC.
In addition to standard frictional and contact constraints and tracking costs, an additional cost function for EE reference tracking from the MICP is included to enhance precision. The NMPC optimization problem is formulated as a Sequential Quadratic Program (SQP) and solved using the OCS2 library \cite{OCS2}, with a time horizon of one second and 100 knot points.

\subsubsection{Whole-Body Control (WBC)}
While NMPC operates at the centroidal level to generate dynamically feasible trajectories, WBC ensures precise execution by resolving full-body state control, including joint torques and contact forces.
The whole-body controller tracks the NMPC trajectory by solving a hierarchical quadratic program (QP) \cite{herzog2016momentum} at 500 Hz. To improve the performance of agile motions such as leaping and jumping, centroidal momentum tracking is included. The state estimator fuses data from the IMU, joint encoders, and motion capture systems to provide accurate body position information. This MPC-WBC hierarchy allows the system to handle both centroidal-dynamics-level and full-body-dynamics-level control in a coordinated manner, ensuring robustness in real-world deployment especially for highly dynamic motions such as jumping.

\subsection{Coordination between Strategy Execution and Tracking Module}\label{sec:coordination}
\begin{figure}
    \centering \includegraphics[width=\linewidth]{multi_threading_new.pdf}
    \caption{Coordination between strategy execution and tracking control module.
    (a) The MICP solving time (denoted by PT) for transitioning from State 1 to State 2 is shorter than the time horizon of the previous reference trajectory (denoted by TT), allowing the seamless appending for the new trajectory.
    (b) The MICP solving time exceeds the time horizon of the previous reference trajectory, requiring the robot to come to a stop (red) and wait for the new trajectory whenever available.}
    \label{fig:micp_mpc_automaton}
\end{figure}
Due to the potential delays in solving MICP during the strategy automaton roll-out, a harmonic coordination between the strategy execution and tracking control module is essential. The tracking module's reference trajectory is updated dynamically alongside the strategy execution process, as shown in Fig.~\ref{fig:micp_mpc_automaton}. The overall process can be summarized as follows:

\subsubsection{Strategy Execution} The strategy automaton execution thread begins by solving the online gait-fixed MICP, starting from State 0 in the automaton. Once the MICP solution is obtained, it immediately sends the reference trajectories and corresponding contact information to the tracking control module. The automaton then progresses to the next transition, using the final condition in the previous trajectory segment as the new initial condition. In Fig.~\ref{fig:micp_mpc_automaton}, the colored blocks in the strategy execution timeline indicate the time taken for each MICP solve during the automaton roll-out. PT and TT denote the planning time and trajectory time, respectively.

\subsubsection{Tracking Control Module}
The MPC-WBC tracking control module receives time-indexed reference trajectories, which can be updated in real-time. After completing the tracking of the current reference trajectory, the robot returns to a stance phase, ready to accept new reference trajectories. As depicted in Fig.~\ref{fig:micp_mpc_automaton}, the colored blocks in the tracking control module represent the time horizon of each reference trajectory sent by the strategy execution thread. Once the initial reference trajectory is generated, the MPC-WBC thread begins tracking it using more accurate dynamics models, as described in Sec.\ref{sec:tracking_control}.

\subsubsection{Delay Handling}
For more complex scenarios involving a larger number of terrain polygons, the MICP solving time may increase and exceed the time horizon of the generated reference trajectory. Fig.~\ref{fig:micp_mpc_automaton}(a) and (b) illustrate two cases of MICP solving times:
Case (a): The solving time for transitioning from automaton State 1 to State 2 is shorter than the time horizon of the previous reference trajectory. In this case, the new reference trajectory is seamlessly appended to the existing one, and the robot continues tracking the previous trajectory.
Case (b): The solving time exceeds the time horizon of the previous reference trajectory, and the robot has already entered a stance phase (red block) when the MICP solution is obtained. In this case, the robot waits until the newly generated reference trajectory is sent based on the current system time (red block in Fig.~\ref{fig:micp_mpc_automaton} (b)).

% \subsubsection{Error Handling and Replanning}
% If the MPC thread predicts a state that reaches the final state but deviates beyond the specified tolerance, the automaton thread resets to this new initial state and reruns the MICP to adjust the plan. If no significant deviation occurs, the automaton thread continues rolling out, using the desired state until the local waypoint is reached.



==> journal_tex/preliminaries.tex <==
\section{Preliminaries}
Let us start with an example to motivate our framework.

% throughout the paper.
\noindent
\textbf{Example~\examplelabel{example:1}}.
% (9-grid locomotion). 
\textit{Consider a 2D grid world with nine cells (yellow) in Fig.~\ref{fig:preliminary_nine_squares}. The robot must move from an initial square (usually the center square) 
to a desired goal square indicated by the star. 
Each cell is assigned a terrain type, such as $\textit{Dense}$ or $\textit{Sparse}$ stepping stones.}

%%%%% Fig. 9 grid %%%%
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{preliminary_drawing.pdf}
    \caption{Terrain abstraction and skill definition. (a) Top-down view of the real-world terrain before abstraction. The red polygons denote the segmented terrain polygons. (b) Abstraction of the terrain and robot's skills (pink) moving from one location to another. (c) Repair process to find a new skill (blue).}
    \label{fig:preliminary_nine_squares}
\end{figure}
%%%%%%%%%%%%%%%


\subsection{Abstractions}\label{sec:preliminaries_abstraction}
We abstract the local environment states and the robot actions into a set of atomic propositions $\ap$.
We partition $\ap$
% $ = \mathcal{I} \cup \mathcal{O}$ 
into sets of inputs $\mathcal{I}$
% $= \{\mathcal{X}_{\rm{cen}}, \mathcal{E}, \mathcal{X}_{\rm{req}}\}$ 
% (``environment" in the two-player game) 
and outputs $\mathcal{O}$
($\ap = \inp \cup \out$).
% (``robot" in the two-player game). 
The inputs $\mathcal{I}$ consist of
the centroidal inputs $\inpcen$,
% which describe the robot's centroidal states,
% $\mathcal{X}_{\rm{cen}}$ of the robot, 
the terrain inputs $\inpterrain$,
% that describe the environment states surrounding the robot,
% $\mathcal{E}$ that surrounds the robot, 
and the request inputs $\inprequest$
% that specify the goal states provided by the higher-level planner or the user
% the requested robot state $\mathcal{X}_{\rm{req}}$ given by a higher-level planner or user input
($\inp = \inpcen \cup \inpterrain \cup \inprequest$).
The centroidal inputs $\inpcen$ describe the robot's centroidal states,
grounding to the robot's centroidal keyframes
defined as $\mathcal{X} = \{x, y\}$, where the translational states $x$ and $y$ are located at the center of each cell based on the Cartesian-space discretization (the yellow cells as shown in Example~\ref{example:1}). 
% A centroidal state $\inpstatecen \subseteq \inpcen$
% We exclude the vertical height of the robot since it can be purely decided by the terrain information. 
%
The terrain inputs $\inpterrain$
characterize the terrains around the robot,
providing abstracted information decided by a terrain mapping function $\mathcal{T}: \mathcal{P} \rightarrow \pi$. For each cell, the terrain mapping function takes in a set of real-world segmented polygons $\mathcal{P}$ (e.g. the red polygons in Fig.~\ref{fig:preliminary_nine_squares}(a)) and returns an abstraction-level terrain type $\pi$ based on the terrain heights
or terrain densities depending on the practical scenario.
% terrain sparsities, or obstacle detection.
% given the classified terrain information: $\mathcal{E} = \{\rm{cT}, \rm{lT}, \rm{rT}, \rm{uT}, \rm{dT}\}$, where $\rm cT$ stands for current terrain, $\rm lT$ stands for left terrain, $\rm rT$ stands for right terrain, $\rm uT$ stands for upper terrain, and $\rm dT$ stands for down terrain. 
% Each environmental input encodes abstracted information about the terrain, 
% such as the height, sparsity, 
% or obstacle detection. 
%
The request inputs $\inprequest$ allow the high-level planner or the user to specify the target robot states.
%
Since the robot can only control the values of centroidal inputs $\inpcen$, 
we also refer to centroidal inputs $\inpcen$ as controllable inputs
and
terrain and request inputs ($\inpterrain\cup \inprequest$) as uncontrollable inputs.
%
In Example~\ref{example:1},
$\inpcen \coloneqq \{x_i, y_j \mid i,j\in \{0, 1, 2\}\}$,
$\inprequest \coloneqq \{v^\textrm{req} \mid v \in \inpcen\}$,
and
$\inpterrain \coloneqq \{\tvar{x_i}{y_j} \mid i,j\in \{0, 1, 2\}, \pi \in \{0, 1\}\}$
where each input $\tvar{x_i}{y_j}$ is 0 iff the terrain $(x_i, y_j)$ is characterized as \textit{Dense stepping stones}, and 1 iff characterized as \textit{Sparse stepping stones}.
%
% A centroidal state $\inpstatecen \subseteq \inpcen$
% is a 
We define 
the
centroidal states $\inpstatecen \subseteq \inpcen$, 
terrain states $\inpstateterrain \subseteq \inpterrain$, 
and request states
$\inpstaterequest \subseteq \inprequest$
as
subsets of 
centroidal inputs $\inpcen$, 
terrain inputs $\inpterrain$, 
and request inputs $\inprequest$,
respectively.
% Thus is the same as the robot states ($\inprequest = \inpcen$).
%
% The requested state $\mathcal{X}_{\rm{req}}$ is defined same as the robot state: $\mathcal{X}_{\rm{req}} = \mathcal{X}_{\rm{cen}}^{\rm{des}}$. 
% One example with only translational centroidal states is shown in Fig.~\ref{fig:cartoon_problem}(a).
%
In Fig.~\ref{fig:preliminary_nine_squares}b,
the centroidal state is $\{x_1, y_1\}$,
the request state is $\{x_0^{\textrm{req}}, y_2^{\textrm{req}}\}$,
and the terrain state is $\{\tvar{x_0}{y_0}=1, \tvar{x_0}{y_1}=1, \tvar{x_0}{y_2}=1, \tvar{x_1}{y_0}=0, \tvar{x_1}{y_1}=0, \tvar{x_1}{y_2}=0, \tvar{x_2}{y_0}=1, \tvar{x_2}{y_1}=1, \tvar{x_2}{y_2}=1\}$. We assume that the request state and terrain state remain unchanged within the local environment until it is updated.

% \qm{To be deleted} Furthermore, we partition the inputs $\inp$ into controllable inputs $\inpsyms$ and uncontrollable inputs $\inpuser$.
% Controllable inputs $\inpsyms$ represent the environment states the robot can control, i.e. the robot's centroidal states ($\inpsyms = \inpcen$).
% Uncontrollable inputs describe the part of the physical world that the robot does not have control over, i.e. 
% the terrain states $\inpterrain$ and the requested goal states $\inprequest$ ($\inpuser = \inpterrain \cup \inprequest$).

The outputs
% aforementioned output propositions 
$\out$ 
represent
% consists of 
the skills 
that allow the robot to transit among centroidal states,
given the corresponding terrain states.
% $\mathcal{A}$, which define the capabilities of transitioning from one keyframe $\mathcal{X}_{\rm cen}$ to another given certain environment $\mathcal{E}$. 
% Following a TAMP-style definition for future repair process, 
A skill $\skill \in \out$
consists of 
a set of preconditions $\skillpre \subseteq 2^{\inpcen \cup \inpterrain}$
from which the skill is allowed to execute,
and a set of postconditions $\skillpost \subseteq 2^{\inpcen}$, the resulting centroidal states after executing the skill.
%
In Example~\ref{example:1},
the skill $\skillcustom{0}$ moves the robot from the middle to the upper terrain grid (Fig.~\ref{fig:preliminary_nine_squares}b).
The precondition of $\skillcustom{0}$ is
$\skillprecustom{\skillcustom{0}} = \{\{x_1, y_1, \tvar{x_1}{y_1}=0, \tvar{x_0}{y_1}=1\}\}$, and
the postcondition is
$\skillpostcustom{\skillcustom{0}} = \{\{x_0, y_1\}\}$. Each skill not only contains the abstraction-level information for defining the transition, but also corresponds to a continuous-level locomotion gait, such as a one-second trotting gait, which is further defined in Sec.~\ref{sec:motion_primitive}. 

%%%% Fig.2 System architecture %%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{system_diagram.pdf}
    \caption{System architecture overview. The solid lines indicate online communication, while dashed lines represent offline processes.$\vg \epsilon$
    }
    \label{fig:system_diagram}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Reactive  Synthesis}
\subsection{Specifications}
We use the Generalized Reactivity(1) (GR(1)) fragment of Linear Temporal Logic (LTL)~\cite{bloem2012synthesis}
% has been widely used 
to encode task specifications.
% ~\cite{bloem2012synthesis}.
% and automatically synthesize the system's transition behaviors. 
GR(1) specifications $\spec$ 
% is constructed from atomic propositions $\pi \in AP$, which is evaluated to be ${\rm True}$ or ${\rm False}$ and 
follow the grammar 
$\spec \: := \var \:|\: \neg\: \spec \:|\: \spec \:\land\: \spec \:|\: \bigcirc\spec \:|\: \square \spec \:|\: \lozenge \spec$,
where $\var \in \ap$ is an atomic proposition,
$\neg$ ``not'' and $\land$ ``and'' are Boolean operators,
and
$\bigcirc$ ``next'',
$\square$ ``always'',
and $\lozenge$ ``eventually''
are temporal operators.
% . Boolean operators $\neg$ ``not'' and $\wedge$ ``and'' in addition to a set of temporal operators $\ocircle$ ``next'', $\mathcal{U}$ ``until'', and $\mathcal{R}$ ``release'', are denoted. To be concise, we omit the derivations of other boolean operators such as $\vee$ ``or'', $\rightarrow$ ``implies'', and $\leftrightarrow$ ``if and only if'', as well as temporal operators $\Diamond\,\varphi$ ``eventually $\varphi$'' and $\square\,\varphi$ ``always $\varphi$''. 
We refer the readers to~\cite{baier2008principles} for a detailed description of LTL.
% A detailed description of LTL can be referred to \cite{baier2008principles}.

GR(1) specifications are expressed in the form of 
$\spec = \envspec \to \sysspec$,
where $\envspec = \envinit \land \envsafety \land \envlive$ 
is the assumptions on the behaviors of the possibly adversarial environment,
and $\sysspec = \sysinit \land \syssafety \land \syslive$
is the guarantee of the robot's behaviors.
% Specifically,
For $\alpha \in \{e, s\}$,
$\alphainit, \alphasafety, \alphalive$
characterize the 
initial conditions,
safety constraints,
and liveness requirements
respectively.
%
We divide the environment safety assumptions $\envsafety$ into skill assumptions $\envsafetynothard$,
which describe the postconditions of the skills (see Sec.~\ref{sec:spec_gen}),
and hard assumptions $\envsafetyhard$ that cannot be modified
($\envsafety = \envsafetynothard \land \envsafetyhard$).
Similarly, we split the safety guarantees $\syssafety$ into skill guarantees $\syssafetynothard$,
which represent the preconditions of the skills,
and hard guarantees $\syssafetyhard$ that cannot be modified
($\syssafety = \syssafetynothard \land \syssafetyhard$).

==> journal_tex/problem_statement.tex <==
\section{Problem Statement}\label{sec:problem_statement}
% Given a set of inputs $\inp = \inpcen \cup \inpterrain \cup \inprequest$ after discretizing the local environment and categorizing the terrain polygons $\mathcal{P}$, and a set of locomotion primitives, 
We aim to solve a decision-making problem of terrain-adaptive locomotion that generates a symbolic strategy $\mathcal{A}$, consisting of physically feasible skills, to safely and reliably navigate the local environment. To achieve this, the following problems must be addressed, spanning symbolic abstraction to motion planning:

\textbf{Problem 1 (Sec.~\ref{sec:preliminaries_abstraction} and Sec.~\ref{sec:reactive_gait_synthesis}):} 
Given a set of predefined request goals and well-structured terrain polygons $\mathcal{P}$, abstract them into a set of inputs $\inp = \inpcen \cup \inpterrain \cup \inprequest$, find necessary and physically-feasible skills and corresponding locomotion gaits, encode and synthesize realizable task specifications.

\textbf{Problem 2 (Sec.~\ref{sec:online_execution}):} 
Given the synthesized strategy $\mathcal{A}$, an online request goal, and online segmented terrain polygons $\mathcal{P}$, 
address potential online execution failures, including real-world terrain discrepancies and unseen terrain types.

==> journal_tex/related_work.tex <==
\section{Related Work}
\subsection{Hierarchical Planning for Terrain-Adaptive Locomotion}
Planning for terrain-adaptive locomotion can be boiled down into solving contact sequence and timing (equivalently gait), location (equivalently foothold), and robot motion (e.g., Center of Mass (CoM) or base pose), given the chosen kinematics/dynamics model and the perceived terrain information. Hierarchical approaches first separately or simultaneously address part of the above problems and then solve for the rest, which allows for higher computational efficiency.  
% Among them, hierarchical approaches commonly separate the foothold from the gait/contact and base pose planning, which allows for higher computational efficiency.
Kinematic footstep planning focuses on the first two problems, neglecting the robot dynamics through graph-based approaches \cite{kolter2008control,kalakrishnan2010fast,winkler2014path,mastalli2015line,fankhauser2018robust,griffin2019footstep} or optimization-based approaches \cite{deits2014footstep,tonneau2020sl1m,risbourg2022real}.
% Another perspective of hierarchical approaches is on planning over a set of actions\cite{kolter2008control,kalakrishnan2010fast,winkler2014path,mastalli2015line,griffin2019footstep}.
Although non-fixed gait/contact plans can be generated for very rough terrains \cite{hauser2005non,hauser2008using,bretl2006motion,tonneau2018efficient}, conservative quasi-static motions are generated for challenging terrains due to the kinematic simplification during  footstep planning. 
% While dynamically-feasible contact plans are also reported in, heavy computational time and difficulty in handling collision avoidance restrict the online re-planning.

Given the recent advances in optimization-based approaches, notably Model Predictive Control (MPC), another focus of the literature is on the local foothold adaptation and the integration of robot dynamics for dynamic locomotion.
Instantaneous foothold adaptation around a nominal location, with a fixed and cyclic gait, is performed based on heuristic search \cite{jenelten2020perceptive,kim2020vision,agrawal2022vision} or learning approaches \cite{magana2019fast, villarreal2020mpc,yu2021visual,gangapurwala2022rloc}. 
In \cite{grandia2021multi,jenelten2022tamols,grandia2023perceptive}, the base pose and foothold are optimized jointly, demonstrating impressive terrain traversing capabilities on rough terrains.
% , which generates dynamically consistent trajectories. 

However, the above dynamic locomotion works consider a fixed gait pattern that usually prohibits achieving versatile behaviors, such as jumping. 
In \cite{Park2015OnlinePF, kim2020vision,gilroy2021autonomous}, jumping motions are generated offline and triggered through heuristics. 
In \cite{fernbach2017kinodynamic,norby2020fast,chignoli2022rapid}, RRT-Connect is used for rapid kino-dynamic locomotion planning, and the switch between normal walking and jumping is either embedded inside a reduced-order model during sampling \cite{norby2020fast} or decided by a pre-trained feasibility classifier \cite{chignoli2022rapid}. 
% The switching mechanism between different gaits is either hardcoded or lacks a formal guarantee of feasibility. 
% The challenges come from trajectory concatenation. On the other hand, model-free approaches have demonstrated the emergence of dynamic gaits reactive to discontinuous terrains \cite{pmlr-v164-margolis22a,hoeller2023anymal}
Beyond limited gait modes, other works focus on online gait planning and/or foothold selection and deploy MPC to track the plan,
% separate the gait pattern and/or foothold selection from robot motion planning, 
which can be further categorized into model-free \cite{da2021learning,yang2022fast,xie2022glide,pmlr-v164-margolis22a,yu2024learning} and model-based methods \cite{boussema2019online,wang2023and,sun2023free}.

\subsection{Simultaneous Planning via Optimization}
Planning for terrain-adaptive locomotion problem can also be formulated as a combinatorial optimization problem that simultaneously optimizes for gait, foothold, and robot dynamics.
One approach is to incorporate rigid \cite{posa2014direct} or smoothed \cite{mordatch2012discovery} complementarity constraints, which accurately model the physical contact interaction behavior but remains computationally inefficient due to the non-smoothness and highly nonlinearity. Promising online MPC results are reported in \cite{aydinoglu2022real,le2024fast,yang2024dynamic} but still limited to low-dimensional system and static environment. 

Another way of encoding discrete contact decisions is to treat both the contact state and the contact plane selection for each leg at each timestep as binary variables \cite{valenzuela2016mixed,shirai2022simultaneous,jiang2023locomotion}. The underlying problem can be formulated as Mixed Integer Program (MIP). Convex approximations of nonlinear dynamics, usually centroidal dynamics, and constraints are typically required to transform the MIP into a more tractable Mixed Integer Convex Program (MICP), albeit with an increased number of binary variables. 
A global certificate for the approximated convex problem exists upon convergence \cite{dai2019global}, providing an ideal means to determine the feasibility in our proposed method.
To relieve the computational burden due to the introduction of many binary variables, the works of \cite{ponton2016convex,ding2020kinodynamic,acosta2023bipedal} assume the contact sequence and timing are chosen \textit{a prior}, and only optimize the contact plane selection. Aceituno-Cabezas et al. \cite{aceituno2017simultaneous} optimize the contact sequence within a certain gait cycle that fixes the number of footsteps. 
However, it is inevitable that the problem complexity grows exponentially when the number of discrete contact options increases along with the time horizon and terrain features. Our work aims to alleviate computational burden through a two-stage approach. In the offline phase, expensive MICPs that optimize both contact state and foothold selection are solved to generate necessary locomotion gaits. In the online phase, efficient MICPs with adaptive and predefined gaits are used to produce dynamically feasible motions and footholds. Additionally, guided by a synthesis-based task planner, each MICP in our work considers shorter time horizons and fewer terrain features compared to solving a single large MICP problem.

% Our approach: between hierarchical planning and combinatorial optimization. Split the contact planning problem into gait and footstep selections, while the gait planner considers dynamical feasibility given the terrain information.

% Different from \cite{shirai2022simultaneous}, this work: 

% 1. Considers the angular evolvement of the robot to allow more versatile motion generation 

% 2. We consider a more complicated centroidal optimization problem which provides higher-fidelity solution back to the MICP 

% 3. We fix the gait selection to allow real-time foothold selection 

 

% Different from the LGP work \cite{toussaint2015logic}: 

% 1. We evaluate the entire course of a trajectory and incorporate the underactuated dynamics, which is hard to be divided into multiple sub-problems. 

% Different from the MCTS \cite{amatucci2022monte}: 

% 1. We mostly care about the computational efficiency and the motion feasibility across a certain course. Therefore, two different choices we made here: 

% 2. Our footstep planner assumes a fixed gait and only determines the foothold locations given the steppable regions. 

% 3. The gait selection in our problem setup stays in a relatively higher level, whereas the MCTS is able to discover and optimize the gait. In other words, the high-level search space in our framework is smaller than MCTS.   

% Independent Gait Scheduling

% As discussed above, simultaneously planning for the gait and the footholds given perception feedback remains a challenging problem. Alternatively, impressive results have been reported by separating the gait scheduling and the foothold selection. The state-of-the-art works that handle gait transitions can be divided into model-free \cite{da2021learning,yang2022fast,xie2022glide,pmlr-v164-margolis22a}... and model-based approaches \cite{boussema2019online,wang2023and,sun2023free}.

\subsection{Task and Motion Planning for Contact-Rich Planning}
% Instead of capturing every discrete option as in general MIP, 
Task and Motion Planning (TAMP) formally defines symbolic-level tasks and searches through a graph of predefined motion primitives that enable feasible symbolic transitions \cite{garrett2021integrated}. For more complex physical contact resoning, Toussaint et al. propose Logic Geometric Programming (LGP) \cite{toussaint2015logic} and embed the high-level
logic representation into the low-level motion planner, demonstrating contact-rich tool-use behaviors \cite{toussaint2018differentiable}
after defining abundant action primitives. 
Building on this, a broader range of motions has been showcased, including versatile manipulation \cite{migimatsu2020object,zhao2021sydebo} and loco-manipulation tasks \cite{sleiman2023versatile}.
In a similar vein, works such as \cite{ding2021hybrid,shirai2021lto,jelavic2021combined,amatucci2022monte,chen2021trajectotree,zhang2023simultaneous,zhu2023efficient,asselmeier2024hierarchical} integrate graph-search or sampling-based methods with optimization-based approaches in a holistic manner, abstracting contact modes within a discrete domain. However, the combinatorial nature of these problems often leads to poor scalability due to the explosion of contact modes. Deploying such approaches online in dynamic environments remains an open challenge. From a different perspective, we abstract a smaller set of task-level contact modes as locomotion gaits over a specific time horizon and distance, allowing the MICP to solve for details such as contact locations and robot motion during execution. This shifts the focus to selecting locomotion gaits within a local environment while ensuring safety and completeness through synthesis-based approaches.

Unlike LGP that solves an integrated TAMP problem, synthesis-based approaches using Linear Temporal Logic (LTL) operate primarily at the task level, emphasizing safety and completeness guarantees within the task domain \cite{kress2018synthesis}. These methods typically synthesize a sequence of task-level actions, which are then executed by a motion planner. Recently, LTL has been applied to safe locomotion tasks, employing distinct task-level abstractions on topological maps of terrain \cite{kulgod2020temporal,zhou2022reactive,jiang2023abstraction} or locomotion keyframes for reduced-order models \cite{gu2022reactive,shamsah2023integrated,zhao2016high,zhao2022reactive}.
Reactive synthesis \cite{pnueli1989synthesis}, widely applied to mobile robots \cite{kress2009temporal}, has been employed to enable prompt decision-making in response to more complex environments \cite{zhao2016high,shamsah2023integrated} or external perturbations \cite{gu2022reactive}. Notably, Zhao et al. \cite{zhao2016high,zhao2022reactive} formulate the terrain-adaptive locomotion problem as a sequential decision-making task, selecting appropriate locomotion modes with predefined contact and locomotion keyframes to accommodate dynamically changing terrains. However, the locomotion mode selection is explicitly encoded in the LTL specification using expert knowledge, lacking a physically feasibility guarantee.
% To reduce the complexity of solving multi-contact, long-horizon, and kino-dynamic planning problems, a single optimization problem can be divided into multiple sub-problems, facilitating faster computation through holistic approaches. Graph-search planning (GSP) or sampling-based planning (SBP) methods have been proposed to be combined with dynamically feasible motion primitives \cite{shkolnik2011bounding, fernbach2017kinodynamic,norby2020fast,shirai2021lto,ding2021hybrid,jelavic2021combined,chignoli2022rapid,amatucci2022monte}. Superior planning speed has been reported with reduced-order models \cite{fernbach2017kinodynamic,norby2020fast,carpentier2018multicontact} or pre-trained feasibility classifier \cite{chignoli2022rapid}. 
% The authors in \cite{zhao2021sydebo,shirai2021lto,ding2021hybrid,jelavic2021combined,amatucci2022monte,chen2021trajectotree,zhang2023simultaneous} fully exploit the robot dynamics through TO combined with a high-level search. 
% Among them, researchers in \cite{jelavic2021combined,amatucci2022monte} explicitly reason the gait/contact mode in the search process. 
% However, the combinatorial nature of the problem renders poor scalability due to the explosion of contact modes. Online deployment of this type of approaches given changing terrain information remains an open problem.
In this work, we aim to combine the strengths of reactive synthesis and MICP, utilizing the global certificate of MICP as a feasibility checker for terrain-adaptive locomotion.

% The lack of immediate reaction and safety guarantee given real-time terrain information still prohibits this type of approach from online deployment.

\subsection{Physically-Feasible Reactive Synthesis}
% Linear Temporal Logic (LTL) serves as a prevalent tool for encoding temporal task specifications and automating the synthesis of system transition behaviors within the robotics community. Originating from its proposal for model checking by Pnueli in 1977 \cite{pnueli1977temporal}, LTL has gained substantial traction in robotics research, initially prevalent in studies involving wheeled robots \cite{kress2009temporal, decastro2018collision}, and more recently, extending to legged robots \cite{warnke2020towards, zhao2022reactive, kulgod2020temporal, gu2022reactive, shamsah2023integrated}.
% Reactive Synthesis, denoting the automated generation of a reactive system to ensure compliance with desired specifications, regardless of external inputs, was introduced by Pnueli in 1989 \cite{pnueli1989synthesis}. Given the escalating complexity associated with lengthy LTL formulas, a subset of LTL, General Reactivity of Rank 1 (GR(1)), was proposed to streamline the synthesis process \cite{piterman2006synthesis}. This subset proves especially beneficial in managing the synthesis process efficiently.

% (Replanning in the task level; BT, TAMP; inflation? Check Jonas paper again) 

% In contrast to Task and Motion Planning (TAMP), a paradigm that typically integrates symbolic search with geometric or optimization-based motion planners, reactive synthesis primarily operates at the task level. 

% Reactive synthesis primarily operates at the task level and involves specifying Linear Temporal Logic (LTL) formulas that encompass sequencing, conditions, and reactions to environmental events. 
While reactive synthesis can promptly and safely respond to dynamic environments, it typically does not assess physical feasibility. To bridge the gap between discrete abstraction and continuous system dynamics, various strategies have been proposed. Some studies \cite{decastro2014dynamics,fainekos2006translating} focus on automatically synthesizing controllers in the continuous domain based on high-level specifications. Another approach involves incorporating dynamics directly into the reactive synthesis process by abstracting physical systems, including nonlinear \cite{bhatia2010sampling}, switched \cite{liu2013synthesis}, and hybrid systems \cite{maly2013iterative} with manageable model complexities. However, for legged robots with multiple contacts navigating dynamic terrains, these physically feasible reactive synthesis approaches remain computationally intractable.

Recent efforts \cite{pacheck2020finding, pacheck2022physically} focus on symbolic repair for unrealizable task specifications, defining symbolic skills with preconditions and postconditions, similar to TAMP, to identify missing skills that make the specification realizable. These works introduce iterative feasibility checks based on symbolic repair suggestions, emphasizing alignment between symbolic task specifications and physical reality. Building on this, Meng et al. \cite{meng2024automated} extends the approach to online symbolic repair.
Inspired by these works, we adopt a similar mechanism for terrain-adaptive locomotion. Specifically, we abstract the robot and terrain states in a local environment and define physically feasible skills by solving MICP. \todo To address scalability issues arising from complex terrain features, we employ a high-level manager to decompose the problem into smaller subproblems, enabling faster repair and synthesis.

% Three main novelties in our reactive planner:

% 1) We leverage the powerfulness of reactive synthesis to  reason about the robot traversability with regard to the terrain information.

% 2) We generate skills that are physically feasible offline; a symbolic repair process is proposed to handle unrealizable specifications.

% 3) We perform fast run-time feasibility checking through graceful coordination toward MPC given real-time robot and environment representations.

==> journal_tex/results.tex <==
\section{Simulation}\label{sec:experiments}
We first present two case studies to demonstrate the synthesis and repair processes in both offline and online phases. Examples of maneuvering over various environments highlight the framework's efficacy and generalizability. Benchmarking experiments are also conducted to further compare our proposed framework with other alternative approaches.
\subsection{Robot Setup}
As mentioned earlier, we verify our algorithms on two separate robot platforms, Unitree Go2 and SkyMul Chotu. The parameters for each robot are defined in Table~\ref{tab:robot_parameter} and used for formulating our optimization problems, including the robot mass $m$, torque limit $\vg \tau_{\text{max}}$ and the reference joint position $\v q_j^{\text{ref}}$ for a single leg with three joints, the reference foot position relative to the base frame $^\mathcal{B} \v p_j^{\text{ref}}$ and the maximum deviation of the foot position $\v p_j^{\text{max}}$ for the front left leg ($j=0$), and the moment of inertia of the approximated single rigid body $\v I$.
\begin{table}[t]
    \caption{Robot Parameters}
    \centering
     \begin{tabular}{c | c | c}
         \hline
         Parameter & Unitree Go2 & SkyMul Chotu\\\hline
         $m (kg)$ & 15.071 & 19.978\\
         $\vg \tau_{\text{max}} (N \cdot m)$ & (23.5, 23.5, 45.4) & (23.5, 23.5, 33.5)\\
         $\v q_j^{\text{ref}}(rad)$ & (0.0, 0.72, -1.44) & (0.0, 0.72, -1.44)\\
         $^\mathcal{B} \v p_j^{\text{ref}}(m)$ & (0.1805, 0.1308, -0.29) & (0.2118, 0.210, -0.30)\\
         $\v p_j^{\text{max}}(m)$ & (0.15, 0.1, 0.15) & (0.15, 0.1, 0.15)\\
         $\v I (kg \cdot m^2)$ & diag(0.152, 0.369, 0.388) & diag(0.396, 0.915, 1.107)\\
         \hline
    \end{tabular}
    \label{tab:robot_parameter}
\end{table}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{offline_terrains.pdf}
    \caption{Four terrain cases used for offline repair in our case study.}
    \label{fig:offline_terrains}
\end{figure}

\subsection{Offline Synthesis and Repair Case Study}
For the purpose of evaluating offline synthesis and repair process, we provide additional set of predefined terrain polygons , which are abstracted into sparse and dense terrain types similar to Example~\ref{example:1}.
Fig.~\ref{fig:offline_terrains} shows four 9-grid terrain combinations with varying stepping stone sparsities. The first row presents the real-world terrain polygons, while the second row displays the corresponding symbolic-level maps. The grid size is chosen based on factors such as robot size and terrain dimensions. In all examples, we use a 0.6 m cell size, but this can be adjusted for practical applications. 
We use a 1.5-second trotting gait as the motion primitive given ahead of time, and the MICP planner has a 0.02s timestep, resulting in $N=75$ knot points, and $R=8$ terrain polygons per transition. In Fig.~\ref{fig:offline_repair}, the pink arrows indicate the original feasible transitions. The robot successfully navigates upward and downward across all terrains; terrain case (a) achieves all transitions and is not shown in the figure due to space limit. 
The infeasible transition arises when moving sideways on sparse stepping stones, restricted by the leg kinematics constraint in Eq.~\ref{eq:rom}. However, specifications for terrain case (b) and (c) remain realizable as the robot avoids sideways movement by taking detour steps, indicating that not all skills are required for these types of  terrains. Such a coincidence does not apply to terrain case (d), where the specification becomes unrealizable due to physically unreachable $(x_1,y_0)$ and $(x_1,y_2)$. This unrealizability triggers a symbolic repair to identify a symbolic suggestion in \todo seconds, adding two additional transitions (blue arrows). By reconfiguring to a bounding gait with short aerial phases, the robot restores transition feasibility, making terrain case (d)'s specification realizable.

% we the offline terrains for specification generation. We use the above case for demonstrating the offline repair. We can emphasize that not all the transitions are needed for navigating to a desired waypoint considering the robot physical feasibility. The robot does not necessarily need to move sideways. It becomes more urgently needed when the state space increases. This also allows us to incorporate strategy in terms of specific terrain combinations. Only exception case is the one with all sparse terrains.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{offline_repair.pdf}
    \caption{Offline repair results for terrain cases (b), (c), and (d) in Fig.~\ref{fig:offline_terrains}. We also illustrate the original trotting and repaired bounding gait.}
    \label{fig:offline_repair}
\end{figure}

\subsection{Online Repair Case Study (\todo update with a new terrain type)}
As a case study to demonstrate the capability of handling unforeseen terrains, we preclude the evaluation for terrain (d). An online scenario is then created as shown in Fig.~\ref{fig:online_repair} with randomized sparsities ranging from 0 to 0.15 m. In Fig.~\ref{fig:online_repair}, the robot is tasked with reaching a global waypoint using a naive global planner to find the shortest path.
%selecting the closest grid in the 9-grid map as the local waypoint. 
Then the local waypoint in the 9-grid map is selected by choosing the closest grid. 
The robot starts to navigate until it encounters an unforeseen terrain case (e) after abstracting the perceived local terrain shapes. Grids $(x0,y0)$ and $(x2,y0)$ are unreachable as shown in Fig.~\ref{fig:online_repair}(e1) since the sideway walking capability between sparse terrains was not captured. Upon detecting such a violation of the environment specification, the online repair is triggered, generating a new dynamically feasible skill for transitions $(x1,y0) \rightarrow (x0,y0)$ and $(x2,y1) \rightarrow (x2,y0)$ in \todo seconds shown in Fig.~\ref{fig:online_repair}(e2). The robot then successfully traverses terrain case (e) and can handle this terrain when encountering it again.

% (Done) Show the online repair result for a certain type of terrain. (Online terrain snapshot $\rightarrow$ polygons considered in the 9-grid $\rightarrow$ abstraction $\rightarrow$ existing skills $\rightarrow$ repaired skills)
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{online_repair.pdf}
    \caption{Online repair results after witnessing unforeseen terrains.}
    \label{fig:online_repair}
\end{figure}

\subsection{Maneuvering Showcase}
To demonstrate the generalizability of the proposed framework, we examine two scenarios with varying complexities, numbers of potential safe stepping regions, and robot platforms.
\subsubsection{Unstructured Terrain}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{online_terrains.pdf}
%     \caption{(Will be updated to have rebar scenario.) Online scenarios with random sparsity of stepping stone and obstacles.}
%     \label{fig:online_terrains}
% \end{figure}
Unlike the case studies, to further study the scalability of the proposed framework, we abstract eight terrain types: \textit{flat terrain}, \textit{high terrain}, \textit{low terrain}, \textit{dense stone}, \textit{sparse stone}, \textit{gap}, \textit{high gap} and \textit{low gap}. The \textit{obstacle} is also explicitly captured as a terrain type and applied to all scenarios. To avoid transitioning to an obstacle grid, we add specifications for obstacle avoidance as hard constraints, and assume the requested waypoint is not an obstacle grid. We create separate scenarios that consider 4 and 8 terrain types selected from the aforementioned terrain types. In addition, the abstracted grid size can be extended to higher resolution and the difference between 3x3 and 5x5 grid size is shown in Fig.~\ref{fig:multiple_sizes}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{5x5_unstructured_demonstration.pdf}
    \caption{Caption}
    \label{fig:multiple_sizes}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{unstructured_8_terrain.pdf}
    \caption{Online scenarios with random sparsity of stepping stone and obstacles.}
    \label{fig:online_terrains}
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{unstructured_randomized.pdf}
%     \caption{Online scenarios with random sparsity of stepping stone and obstacles.}
%     \label{fig:online_terrains_2}
% \end{figure*}

Unstructured - 4 types: flat terrain, dense stepping stone, sparse stepping stone, gap.

% Unstructured - 6 types: flat terrain, high terrain, low terrain, gap, high gap, low gap. 

Unstructured - 8 types: all terrain types included.

Fig.~\ref{fig:online_terrains} illustrates two unstructured scenarios, along with snapshots of the robot traversing these terrains.

\subsubsection{Rebar}
Inspired by the labor-intensive rebar tying task on construction sites that has been studied in previous work \cite{asselmeier2024hierarchical}, we explore a second application where the quadrupedal robot navigates a rebar mat. Each rebar is modeled as a rectangular polygon with a 3 cm width, with spacing ranging from 0.15 to 0.3 m. Unlike the stepping stone scenario, this setup offers more potential stepping regions due to the higher rebar density. The terrain is abstracted into \textit{flat terrain}, \textit{dense rebar}, \textit{sparse rebar}, and \textit{obstacle}.

Rebar - 7 types:

Rebar - 14 types:



Fig.~\ref{fig:rebar-traversing} illustrates the rebar scenario.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{rebar_demonstration.pdf}
    \caption{Caption}
    \label{fig:rebar-traversing}
\end{figure*}

\todo Show the computational time for offline synthesis.

\todo Show the online computation speed for MICP.
\begin{table*}[t]
    \caption{Online MICP Solving Time}
    \centering
     \begin{tabular}{c | c | c | c | c | c | c}
         \hline
         Scenario & Collision Avoidance & Binary Variables & Continuous Variables & Number of Polygons & Solve Time\\\hline
         Unstructured - 4 & No \\
         & Yes \\\hline
         Unstructured - 8 & Yes \\
         & No \\\hline
         Rebar - 7 & No\\
         \hline
         Rebar - 14 & No\\
         \hline
    \end{tabular}
    \label{tab:micp_speed}
\end{table*}

% \todo Show the successful rate of navigation

\subsection{Benchmark: Graph Search-Based Planner}
Larger scenario with longer-horizon planning.

Total planning time, times of gait-fixed MICP and gait-free MICP being solved, times of online repair being triggered.

\subsection{Extensions}\label{sec:extension}
To showcase the flexibility of our framework, we provide two extensions to the existing task-level abstraction.
\subsubsection{Diagonal Movement}\label{sec:extension_diag}

\subsubsection{Yaw Command}\label{sec:extension_yaw}

